Global Optimization via Optimal Decision Trees

The global optimization literature places large emphasis on reducing intractable optimization problems into more tractable structured optimization forms. In order to achieve this goal, many existing methods are restricted to optimization over explicit constraints and objectives that use a subset of possible mathematical primitives. These are limiting in real-world contexts where more general explicit and black box constraints appear. Leveraging the dramatic speed improvements in mixed-integer optimization (MIO) and recent research in machine learning, we propose a new method to learn MIO-compatible approximations of global optimization problems using optimal decision trees with hyperplanes (OCT-Hs). This constraint learning approach only requires a bounded variable domain, and can address both explicit and inexplicit constraints. We solve the MIO approximation efficiently to find a near-optimal, near-feasible solution to the global optimization problem. We further improve the solution using a series of projected gradient descent iterations. We test the method on a number of numerical benchmarks from the literature as well as real-world design problems, demonstrating its promise in finding global optima efficiently.

==> bench_descriptions.tex <==
\begin{center}
    \begin{table}[!h]
        \begin{tabular}{|c|c|}
            Problem name &  Problem description \\
            \hline
            \texttt{himmel16} & Maximize the area of a hexagon of maximum diameter 1.\\
            \hline
            \texttt{kall\_circles\_c6b} & \stackedcell[c]{Find the minimum area of a set of rectangular stock \\ from which to cut a set of circles.}\\
            \hline
            \texttt{pointpack08} & \stackedcell[c]{Find the maximum radius of 8 non-overlapping circles \\ that all lie in the unit-box.}\\
            \hline
            \texttt{flay05h} & \stackedcell[c]{Determine the optimal length and width of rectangular \\ patches of fixed area, so that perimeter is minimized.}\\
            \hline
            \texttt{fo9} & \stackedcell[c]{Optimize a block layout design \\problem with unequal areas.} \\
            \hline
            \texttt{o9\_ar4\_1} & \stackedcell[c]{Optimize a block layout design \\problem with unequal areas.} \\
            \hline
        \end{tabular}
    \caption{The larger benchmark descriptions.}
    \label{tab:largebenchdescriptions}
\end{table}
\end{center}

==> convex.tex <==
CONVEXITY DETECTION

\subsubsection{Convexity detection}

TODO: WRITE ANOTHER PAPER ON THIS TOPIC. REMOVE FROM PAPER LATER. 

In addition, if we can compute the gradient of an explicit constraint via \gls{ad}, we can attempt to detect the convexity of the constraint. This would allow us to avoid decision trees altogether and solve over the constraint using cutting planes. We use the gradients at each sample and \gls{knn}-based heuristics to approximate the local and global convexity of the constraints. For a constraint over $m$ variables, we build a \gls{knn} tree with $2m+1$ points in each cluster, centered at each sample. We compute the local curvature of each cluster by seeing whether the gradient at the center sample is a local under-approximator of the actual function value. Then we assign a value in $\{-1, 0, 1\}^n$ for each sample, depending on whether it is an over-, mixed-, or under- approximator of the local data, corresponding to our approximation of the sign of the Hessian at that point. If we compute that all points have gradients that are local under-approximators, we assume that the function is convex. However, first we perform a final random convexity check, since some pathological function classes may have all points with gradients being local under-approximators, as seen in the Figure~\ref{fig:pathcase}.

\begin{algorithm}[h!]
\caption{Convexity detection}
\label{alg:convex}
\KwResult{Approximate global and local convexity properties of the function.}
Compute gradients at all points: $\Delta = \rm{gradient}(\bx, \by)$ \;
Find $k = 2m+1$ nearest neighbors: $\mathbf{\xi} = \{k\mathrm{NN}(\bx_{i},~ \bx),~\forall i \in [n_{\rm{samples}}]$ \}\;
Initialize convexity vector: $\bh = {0}^n$\;
 \For{$i \in [n]$:}{
    \If{$y_{j} \geq y_{i} + \Delta_i^{\top}(\bx_j - \bx_i),~\forall j \in \xi_{i}$} {
        Locally convex: $h_i = 1$.
        } 
    \ElseIf{$y_{j} \leq y_{i} + \Delta_i^{\top}(\bx_j - \bx_i),~\forall j \in \xi_{i}$}{
        Locally concave: $h_i = -1$.
    }
} 
\end{algorithm}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/pathcase.jpg}
    \caption{Univariate case $f(x) = \min((x-1)^2, (x+2)^2$) in domain $x \in [-5, 10]$, we can show how certain functions are not convex, but look convex locally. }
    \label{fig:pathcase}
\end{figure}
